A Software-based Low-Jitter Servo Clock for Inexpensive Phasor Measurement Units

This paper presents the design and the implementation of a servo-clock (SC) for low-cost Phasor Measurement Units (PMUs). The SC relies on a classic Proportional Integral (PI) controller, which has been properly tuned to minimize the synchronization error due to the local oscillator triggering the on-board timer. The SC has been implemented into a PMU prototype developed within the OpenPMU project using a BeagleBone Black (BBB) board. The distinctive feature of the proposed solution is its ability to track an input Pulse-Per-Second (PPS) reference with good long-term stability and with no need for specific on-board synchronization circuitry. Indeed, the SC implementation relies only on one co-processor for real-time application and requires just an input PPS signal that could be distributed from a single substation clock.

==> analysis.tex <==
\section{Model Description and PI Controller design} %something like that
\label{sec:model}

%For the clarity of the presentation, all the software is written
%taking as reference model the classic servo clock
%design~\cite{someone!}. The controller is a classic PI regulator,
%resulting in a second order system that can be tuned to filter out the
%scillation and noise on the input.  From the implementation point of
%view, the clock is implemented by means of an hardware timer, which
%shows non-idealities due to the use of discretized time periods, but
%also advantages over software--based clocks as the improved time
%resolution with respect to the signal generation.  Of course the
%entire system can be seen as a multi-rate system, with the accumulator
%that runs faster than the controller, because of the discretized
%availability of the time reference (once per second usually,
%henceforth denoted with $T_m$).  

The SC shown in Fig.~\ref{fig:implementation} can be modeled as a
discrete-time liner system discretized at 1 Hz.  The corresponding
block diagram is depicted in Fig.~\ref{fig:model}(a). As described in
the rest of this section, this model can be easily reduced to the
classic SC model shown in Fig.~\ref{fig:model}(b), by considering
explicitly the effect of the accumulator on the reference PPS signal.
%(i.e., the first element in the direct chain).
%-%
\begin{figure}[t]
	\centering 
	\begin{tabular}{c}
		\includegraphics[page=3, trim={3.3cm 5.5cm 3cm 5.5cm}, clip, width=\columnwidth]{../figures/models} \\
		(a) \\
		\includegraphics[page=1, trim={6cm 6.5cm 6cm 6.7cm}, clip, width=0.85\columnwidth]{../figures/models} \\
		(b)
	\end{tabular}
	\caption{Equivalent models of the implemented SC before (a) and after (b) simplification.}
	\label{fig:model}
\end{figure}
%-%
%
%\subsection{Servo Clock model}
%\label{SC_model}

Based on the simplified equivalent model in Fig.~\ref{fig:model}(b), 
%the discrete-time SC can be modeled 
the SC in the $z$-domain basically consists of two subsystems, i.e. 
the clock itself, whose transfer function is 
\begin{equation}
C(z) = \frac{1}{z-1} , %\frac{t_c(z)}{u(z)} 
\label{eq:clock}
\end{equation}
and the PI controller, which can be obtained from the classic backward integration
\begin{equation}
P(z) = K_P + K_I \frac{z}{z-1} , %\frac{u(z)}{e(z)} = 
\label{eq:control}
\end{equation}
where $K_P$ and $K_I$ are the proportional and integral gains,
respectively.  As a consequence, the stability of the closed loop SC
system is related to the closed loop transfer function
\begin{equation}
H(z)=\frac{P(z)C(z)}{1+P(z)C(z)} =  \frac{(z-1)K_P + zK_I}{(z-1)^2 + (z-1)K_P + zK_I} .
\label{eq:cltf}
\end{equation}

The PI controller parameters $K_P$ and $K_I$ in~\eqref{eq:control}
should be tuned in order to meet the desired performance requirements,
such as smallest convergence time or output uncertainty reduction.  To
this end, we represent the relations in~\eqref{eq:clock},
\eqref{eq:control} and~\eqref{eq:cltf} using difference equations.

Let $\tau_m^r(k)$ be the period of the input PPS reference signal in
input (see Fig.~\ref{fig:model}-a) at time $k T_m$, given by the sum
of the ideal period PPS $T_m$ (i.e. 1 s) and jitter $\nu^r(k)$.  The
superscript $r$ stand for ``time reference'', hence all the quantities
are measured in seconds.  The time synchronization error $e^r(k)$,
obtained from the accumulation of the differences between the PPS
reference period $\tau_m^r(k)$ and the PPS local period $\tau_c^r(k)$,
follows the following updating rule:
\begin{equation}
\label{eq:error1}
e^r(k) = e^r(k-1) + \tau_m^r(k) - \tau_c^r(k) ,
\end{equation}
where 
\begin{equation}
\label{eq:TauM}
\tau_m^r(k) = t(k) - t(k-1) + \nu(k) = T_m + \nu^r(k), 
\end{equation}
$t(k)$ is the ideal reference time and, similarly, $\tau_c^r(k)$ is
the time measured by the SC between the period $kT_m$ and $(k-1)T_m$.

As stated in Section~\ref{sec:implementation}, we recall that the
system at hand is a multi-rate system, i.e. the resolution of the
error measurements are given by $1/f_{XO}$, with $f_{XO} = 200$~MHz,
while the resolution of the local clock is $1/f_{c}$, with $f_c =
12.8$~KHz.  We therefore express the previous quantities in ticks
accumulated by the respective clock, rather than in time.  To this
end, lest us define with $n_t$ the number of ticks accumulated in the
reference for every period of the SC, i.e.
\[
n_t = \frac{f_{XO}}{f_c} .
\]
The dynamic of the SC in each and every period of $T_m$ can be instead
represented by
\[
\tau_c(k+1) = b \tau (1 + \alpha) + b \eta(k) + b u(k) ,
\]
where $b = 1/n_t$, $\tau$ is the nominal period (in terms of number of
ticks) accumulated by the SC in every period $T_m$, $\alpha$ is the
relative frequency offset of $f_c$, $\eta(k)$ represents the jitter of
the SC accumulated during $T_m$ and, finally, $u(k)$ is the control
action. Notice that except for $\tau_c(k)$, all the other quantities
are expressed in the oscillator frequency $f_{XO}$.  Moreover, all the
quantities in ticks are denoted without the superscript $r$.  For what
concerns the error, it can be easily shown that
%we immediately have from~\eqref{eq:error1}
\[
e(k+1) = e(k) + \tau_m(k) - n_t \tau_c(k) ,
\]
while for the control action
\[
u(k+1) = u(k) + K_P(e(k+1) - e(k)) + K_I e(k+1) .
\]
By denoting with the vector $q(k) = [e(k), \tau_c(k), u(k)]^T$ the
aggregated state of the system in closed loop, with initial conditions
$q(0) = [0, \tau_c(0), 0]^T$, we can rewrite more compactly the
previous equations as
\[
q(k+1) = A q(k) + G \tau_m(k) + C \eta(k) + F \tau ,
\]
where
\[
A = \begin{bmatrix}
1 & n_t & 0 \\
b K_I & -(K_P + K_I) & b \\
K_I & -n_t (K_P + K_I) & 1
\end{bmatrix},\,\,\,
G = \begin{bmatrix}
1 \\
b (K_P + K_I) \\
K_P + K_I
\end{bmatrix} ,
\]
\[
C = \begin{bmatrix}
0 \\
b \\
0
\end{bmatrix}\,\,\, \mbox{and}\,\,\,
F = \begin{bmatrix}
0 \\
b (1 + \alpha) \\
0
\end{bmatrix} .
\]

Since $q(k+1)$ is a random vector, its mean value is given by
\[
\E{q(k+1)} = A \E{q(k)} + G \E{\tau_m(k)} + F\tau ,
\]
where %from~\eqref{eq:TauM} we have immediately that $\E{\tau_m(k)} =
%t_m(k) - t_m(k-1)$.  
$\E{\cdot}$ denotes the expectation operator.  To compute
the uncertainty of $q(k+1)$ generated by the joint effect of $\nu(k)$
and $\eta(k)$, to a first approximation, we assume that: % we first make the following simplifying assumptions:
$\nu(k)\sim\mathcal{N}(0, \sigma_\nu^2)$, $\eta(k)\sim\mathcal{N}(0,
\sigma_\eta^2)$. 
%and both the noise processes are strict sense
%stationary.  
As a result, the covariance matrix of $q(k+1)$ is given by
\begin{equation}
\label{eq:CovFirst}
%\begin{aligned}
%& Q(k+1) = \\
%& \E{\left (q(k+1) - \E{q(k+1)} \right ) \left (q(k+1) -
%	\E{q(k+1)} \right )^T} = \\
%& \E{\left (A \tilde q(k) + G \nu(k) + C \eta(k) \right ) \left
%	(A \tilde q(k) + G \nu(k) + C \eta(k) \right )^T} = \\
%& A Q(k) A^T + G G^T \sigma_\nu^2 + C C^T \sigma_\nu^2 .
%\end{aligned}
%\begin{aligned}
 Q(k+1) = A Q(k) A^T + G G^T \sigma_\nu^2 + C C^T \sigma_\eta^2 .
%& \E{\left (q(k+1) - \E{q(k+1)} \right ) \left (q(k+1) -
%	\E{q(k+1)} \right )^T} = \\
%& \E{\left (A \tilde q(k) + G \nu(k) + C \eta(k) \right ) \left
%	(A \tilde q(k) + G \nu(k) + C \eta(k) \right )^T} = \\
%& 
%\end{aligned}
\end{equation}
Of course, if the Gaussianity and/or the whiteness property of the input quantities do not
hold, \eqref{eq:CovFirst} holds only approximately. Notice that, by
setting $Q(0)$,~\eqref{eq:CovFirst} can be used to compute
the uncertainty of the state vector
%expresses the time behavior of the
in closed form.

If the parameters are chosen to make~\eqref{eq:cltf} 
stable,~\eqref{eq:CovFirst} can reach a steady-state
equilibrium, i.e., there exists a sufficiently large value $\bar k$ such
that $Q(k+1) = Q(k)$, $\forall k > \bar k$.  Moreover, the variance of the 
SC jitter over 1 s 
%affecting uncertainty of the SC 
is equivalent to the steady-state value of $\E{(e(k) -
	\E{e(k)})^2}$, which is the entry (1,1) of $Q(k)$.
As a consequence, by computing the equilibrium of~\eqref{eq:CovFirst}
and considering only the first entry, it follows that
\begin{equation}
\label{eq:Variance}
\E{(e(k) - \E{e(k)})^2} = \frac{2 (\sigma_\nu^2 + \sigma_\eta^2)}{K_P
	(4 - K_I - 2 K_P)} .
\end{equation}
Combining this equation with the constraints $K_P > 0$, $K_I > 0$ (for
the system stability) and $\E{(e(k) - \E{e(k)})^2} > 0$, it immediately follows that
\[
0 < K_P < 2\,\,\, \mbox{and}\,\,\, K_I < 4 - 2 K_P .
\]
Within this region, $\E{(e(k) - \E{e(k)})^2}$ is minimized once the
denominator  is maximized.  Suitable values for these parameters are visible in Fig.~\ref{fig:Ki_Kp}.
%-%
\begin{figure}[t]
	\centering 
	\includegraphics[width=\columnwidth]{../figures/Ki_Kp}
	\caption{Possible choices of $K_P$ and $K_I$ that stabilize the
		system, with the related value of the denominator
		of~\eqref{eq:Variance}.}
	\label{fig:Ki_Kp}
\end{figure}
%-%
From this analysis, it follows that if a prompt response is needed, a
dead-beat controller with $K_P = K_I = 1$ is needed.  Otherwise, if
the uncertainty has to be minimized, $K_P = 1$ and $K_I = \varepsilon
> 0$ is the right choice, with $\varepsilon$ being a sufficiently small
constant.  Notice, however, that the smaller is $K_I$, the longer is
the convergence time.



==> servoclock.tex <==


\section{Platform description}

% here details on BBB-PRU
% also something on openPMU
% cos`i si da un quadro d' insieme sui constraint e l'ottica del lavoro
% DA TENERE A LIVELLO ABBASTANZA ASTRATTO !!!

% block diagram of disciplined/sync/adc

 Synchronization is traditionally performed with PLLs locking on a reference signal, achieving high performance with hardware PLLs. Nevertheless the use of such components can be avoided, using a servo clock, able to achieve comparable performances on software.
Thanks to such implementation, it is easy to provide synchronization in many application field that require it, with just the effort of writing good code.


%platform description ancora?
%Laverty aggiunge e sistema qualcosa qui
%

